Exploring Pretraining via Active Forgetting for Improving Cross Lingual Transfer for Decoder Language Models

Large Language Models (LLMs) demonstrate exceptional capabilities in a multitude of NLP tasks. However, the efficacy of such models to languages other than English is often limited. Prior works have shown that encoder-only models such as BERT or XLM-RoBERTa show impressive cross lingual transfer of their capabilities from English to other languages. In this work, we propose a pretraining strategy that uses active forgetting to achieve similar cross lingual transfer in decoder-only LLMs. We show that LLMs pretrained with active forgetting are highly effective when adapting to new and unseen languages. Through extensive experimentation, we find that LLMs pretrained with active forgetting are able to learn better multilingual representations which translates to better performance in many downstream tasks.

==> tables/full_belebele.tex <==
\begin{table}
\small
\centering
\begin{tabular}{lrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrr}
\toprule
Model & af & ar & as & bg & bn & cs & da & de & en & es & fi & fr & gu & he & hi & hr & id & it & ja & ko & ml & mr & nb & nl & pt & ru & sv & sw & ta & te & th & tr & ur & vi & zh & $\mu_\text{pretraining}$ & $\mu_\text{adapting}$ & $\mu_\text{other}$ & $\mu_\text{overall}$ \\
\midrule
\multicolumn{40}{c}{Number of parameters = 400M}\\
\midrule
Baseline & \bfseries 0.118 & \bfseries 0.174 & \bfseries 0.131 & \bfseries 0.136 & 0.067 & 0.119 & 0.056 & 0.096 & \bfseries 0.118 & \bfseries 0.135 & 0.091 & 0.133 & 0.125 & 0.080 & \bfseries 0.159 & 0.099 & 0.045 & 0.118 & 0.139 & 0.101 & 0.121 & 0.074 & 0.040 & 0.075 & \bfseries 0.151 & \bfseries 0.151 & \bfseries 0.106 & 0.062 & \bfseries 0.137 & 0.118 & 0.144 & 0.135 & 0.069 & 0.053 & \bfseries 0.081 & \bfseries 0.117 & 0.113 & 0.095 & 0.107\\
BA & 0.066 & 0.091 & 0.073 & 0.108 & 0.075 & \bfseries 0.121 & 0.080 & 0.061 & 0.063 & 0.103 & 0.047 & 0.098 & 0.159 & \bfseries 0.081 & 0.075 & 0.107 & 0.109 & 0.074 & \bfseries 0.164 & 0.126 & 0.059 & \bfseries 0.158 & \bfseries 0.123 & 0.078 & 0.095 & 0.045 & 0.098 & \bfseries 0.086 & 0.100 & 0.114 & 0.057 & 0.065 & \bfseries 0.111 & \bfseries 0.085 & 0.043 & 0.075 & 0.108 & 0.092 & 0.091\\
AFA & 0.063 & 0.117 & 0.074 & 0.100 & \bfseries 0.151 & 0.077 & \bfseries 0.122 & \bfseries 0.140 & 0.112 & 0.079 & \bfseries 0.099 & \bfseries 0.142 & \bfseries 0.160 & 0.081 & 0.046 & \bfseries 0.127 & \bfseries 0.114 & \bfseries 0.125 & 0.118 & \bfseries 0.138 & \bfseries 0.151 & 0.086 & 0.104 & \bfseries 0.136 & 0.067 & 0.101 & 0.059 & 0.080 & 0.128 & \bfseries 0.157 & \bfseries 0.177 & \bfseries 0.187 & 0.085 & 0.085 & 0.073 & 0.090 & \bfseries 0.133 & \bfseries 0.110 & \bfseries 0.110\\
\midrule
\multicolumn{40}{c}{Number of parameters = 782M}\\
\midrule
Baseline & 0.145 & \bfseries 0.169 & 0.125 & 0.130 & \bfseries 0.161 & 0.115 & 0.203 & 0.186 & \bfseries 0.148 & \bfseries 0.136 & 0.124 & 0.137 & 0.154 & \bfseries 0.183 & \bfseries 0.148 & \bfseries 0.170 & 0.169 & \bfseries 0.180 & 0.181 & 0.150 & \bfseries 0.197 & 0.155 & 0.167 & 0.152 & 0.118 & \bfseries 0.210 & \bfseries 0.181 & 0.147 & \bfseries 0.180 & 0.146 & 0.165 & 0.168 & 0.122 & 0.126 & \bfseries 0.196 & \bfseries 0.160 & 0.158 & 0.157 & 0.158\\
BA & 0.129 & 0.169 & \bfseries 0.147 & 0.112 & 0.151 & 0.138 & \bfseries 0.211 & 0.127 & 0.131 & 0.106 & 0.133 & 0.180 & \bfseries 0.183 & 0.089 & 0.100 & 0.105 & \bfseries 0.184 & 0.111 & 0.168 & 0.156 & 0.144 & 0.168 & 0.130 & \bfseries 0.205 & 0.215 & 0.101 & 0.142 & 0.096 & 0.168 & 0.120 & 0.152 & \bfseries 0.241 & 0.163 & 0.115 & 0.134 & 0.119 & 0.188 & 0.138 & 0.146\\
AFA & \bfseries 0.189 & 0.133 & 0.127 & \bfseries 0.171 & 0.149 & \bfseries 0.164 & 0.187 & \bfseries 0.191 & 0.131 & 0.111 & \bfseries 0.178 & \bfseries 0.226 & 0.175 & 0.166 & 0.126 & 0.127 & 0.146 & 0.141 & \bfseries 0.194 & \bfseries 0.254 & 0.146 & \bfseries 0.221 & \bfseries 0.173 & 0.166 & \bfseries 0.228 & 0.121 & 0.159 & \bfseries 0.166 & 0.163 & \bfseries 0.186 & \bfseries 0.215 & 0.239 & \bfseries 0.212 & \bfseries 0.185 & 0.192 & 0.148 & \bfseries 0.211 & \bfseries 0.166 & \bfseries 0.173\\
\midrule
\multicolumn{40}{c}{Number of parameters = 1.6B}\\
\midrule
Baseline & 0.201 & \bfseries 0.181 & \bfseries 0.223 & 0.167 & \bfseries 0.212 & 0.151 & 0.201 & 0.196 & \bfseries 0.241 & 0.177 & 0.153 & 0.241 & 0.168 & \bfseries 0.228 & \bfseries 0.234 & 0.207 & 0.152 & 0.157 & 0.191 & 0.249 & 0.191 & 0.210 & 0.159 & 0.208 & 0.178 & 0.150 & \bfseries 0.250 & \bfseries 0.167 & \bfseries 0.177 & \bfseries 0.226 & 0.175 & 0.165 & \bfseries 0.222 & \bfseries 0.195 & 0.185 & \bfseries 0.184 & 0.199 & 0.198 & 0.194\\
BA & 0.136 & 0.137 & 0.140 & 0.131 & 0.177 & 0.140 & \bfseries 0.319 & 0.196 & 0.211 & 0.175 & 0.174 & 0.207 & 0.238 & 0.203 & 0.145 & 0.195 & 0.174 & \bfseries 0.181 & 0.271 & \bfseries 0.280 & 0.150 & 0.197 & 0.143 & \bfseries 0.231 & \bfseries 0.218 & 0.135 & 0.180 & 0.142 & 0.117 & 0.143 & \bfseries 0.211 & 0.187 & 0.161 & 0.144 & 0.197 & 0.167 & 0.236 & 0.156 & 0.182\\
AFA & \bfseries 0.251 & 0.172 & 0.185 & \bfseries 0.187 & 0.195 & \bfseries 0.185 & 0.214 & \bfseries 0.213 & 0.144 & \bfseries 0.211 & \bfseries 0.207 & \bfseries 0.281 & \bfseries 0.275 & 0.202 & 0.179 & \bfseries 0.213 & \bfseries 0.224 & 0.173 & \bfseries 0.325 & 0.276 & \bfseries 0.217 & \bfseries 0.225 & \bfseries 0.214 & 0.201 & 0.185 & \bfseries 0.160 & 0.242 & 0.162 & 0.160 & 0.207 & 0.205 & \bfseries 0.222 & 0.184 & 0.187 & \bfseries 0.224 & 0.184 & \bfseries 0.241 & \bfseries 0.206 & \bfseries 0.209\\
\bottomrule
\end{tabular}
\caption{Language-wise results on belebele  \citep{bandarkar2023belebele}. BA refers to Baseline adapted model. AFA refers to Active Forgetting adapted model. $\mu_\text{pretraining}$ refers to performance averaged over languages in the pretraining split. $\mu_\text{adapting}$ refers to averaging over languages in the adapting split. $\mu_\text{other}$ refers to averaging on languages that are in neither split. $\mu_\text{overall}$ refers to the average over all languages.}
\label{tab:full_belebele}
\end{table}

==> tables/full_isotropy.tex <==
\begin{table}
\small
\centering
\begin{tabular}{lrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrr}
\toprule
Model & af & ar & az & bg & bn & co & cs & da & de & en & es & et & fi & fr & gu & ha & he & hi & hu & id & it & iw & ja & ka & ko & ml & mn & mr & my & nl & no & pl & ps & pt & ru & se & sk & sq & sr & st & sv & sw & ta & te & tg & th & tr & ur & vi & zh & $\mu_\text{pretraining}$ & $\mu_\text{adapting}$ & $\mu_\text{other}$ & $\mu_\text{overall}$ \\
\midrule
\multicolumn{55}{c}{Number of parameters = 400M}\\
\midrule
Baseline & 0.605 & 0.634 & \bfseries 0.676 & \bfseries 0.581 & \bfseries 0.630 & 0.741 & 0.692 & 0.711 & \bfseries 0.630 & 0.674 & 0.635 & 0.730 & 0.740 & 0.703 & 0.723 & 0.693 & \bfseries 0.670 & 0.714 & 0.728 & 0.805 & 0.689 & 0.679 & \bfseries 0.616 & 0.722 & 0.693 & \bfseries 0.575 & 0.639 & 0.694 & 0.663 & \bfseries 0.566 & 0.647 & \bfseries 0.628 & \bfseries 0.679 & 0.693 & 0.780 & 0.669 & 0.745 & 0.707 & 0.649 & 0.688 & \bfseries 0.674 & 0.641 & 0.665 & \bfseries 0.639 & \bfseries 0.596 & \bfseries 0.560 & 0.650 & 0.647 & 0.683 & \bfseries 0.600 & 0.683 & 0.663 & 0.667 & 0.670\\
BA & 0.695 & \bfseries 0.566 & 0.741 & 0.610 & 0.646 & 0.693 & \bfseries 0.681 & \bfseries 0.654 & 0.695 & 0.656 & 0.603 & 0.685 & 0.658 & 0.712 & 0.732 & 0.688 & 0.698 & 0.754 & 0.642 & 0.651 & 0.683 & 0.663 & 0.634 & 0.740 & 0.665 & 0.688 & 0.703 & \bfseries 0.655 & 0.697 & 0.577 & 0.661 & 0.715 & 0.715 & 0.656 & \bfseries 0.673 & \bfseries 0.548 & 0.687 & 0.642 & 0.636 & \bfseries 0.672 & 0.734 & \bfseries 0.585 & \bfseries 0.662 & 0.744 & 0.620 & 0.699 & 0.564 & \bfseries 0.622 & 0.625 & 0.662 & 0.659 & 0.651 & 0.678 & 0.666\\
AFA & \bfseries 0.581 & 0.588 & 0.742 & 0.619 & 0.639 & \bfseries 0.636 & 0.685 & 0.687 & 0.693 & \bfseries 0.653 & \bfseries 0.569 & \bfseries 0.684 & \bfseries 0.545 & \bfseries 0.576 & \bfseries 0.571 & \bfseries 0.630 & 0.690 & \bfseries 0.688 & \bfseries 0.621 & \bfseries 0.649 & \bfseries 0.613 & \bfseries 0.624 & 0.627 & \bfseries 0.630 & \bfseries 0.598 & 0.591 & \bfseries 0.601 & 0.767 & \bfseries 0.526 & 0.615 & \bfseries 0.628 & 0.672 & 0.686 & \bfseries 0.589 & 0.673 & 0.667 & \bfseries 0.680 & \bfseries 0.628 & \bfseries 0.543 & 0.696 & 0.803 & 0.653 & 0.693 & 0.668 & 0.623 & 0.570 & \bfseries 0.550 & 0.627 & \bfseries 0.559 & 0.637 & \bfseries 0.640 & \bfseries 0.624 & \bfseries 0.640 & \bfseries 0.636\\
\midrule
\multicolumn{55}{c}{Number of parameters = 782M}\\
\midrule
Baseline & 0.588 & 0.576 & 0.639 & 0.554 & 0.621 & 0.647 & 0.657 & 0.631 & \bfseries 0.618 & 0.610 & 0.555 & 0.651 & 0.659 & 0.621 & 0.622 & 0.642 & \bfseries 0.582 & 0.626 & 0.641 & 0.699 & 0.588 & 0.612 & 0.592 & 0.632 & 0.604 & 0.568 & 0.563 & 0.651 & 0.565 & \bfseries 0.523 & 0.617 & 0.610 & \bfseries 0.624 & 0.627 & 0.683 & 0.615 & 0.667 & 0.673 & 0.576 & \bfseries 0.603 & 0.667 & 0.580 & 0.618 & 0.588 & \bfseries 0.542 & 0.550 & 0.589 & 0.580 & 0.594 & \bfseries 0.559 & 0.610 & 0.607 & 0.612 & 0.610\\
BA & 0.591 & 0.547 & 0.705 & \bfseries 0.542 & 0.592 & 0.654 & 0.604 & 0.616 & 0.631 & 0.615 & 0.537 & \bfseries 0.626 & 0.604 & 0.619 & 0.653 & 0.622 & 0.628 & 0.667 & 0.607 & 0.596 & 0.597 & 0.653 & \bfseries 0.562 & 0.676 & 0.598 & 0.620 & 0.591 & \bfseries 0.618 & 0.638 & 0.530 & 0.617 & \bfseries 0.600 & 0.661 & 0.610 & 0.639 & \bfseries 0.531 & \bfseries 0.600 & 0.600 & 0.611 & 0.643 & \bfseries 0.611 & \bfseries 0.562 & \bfseries 0.589 & 0.680 & 0.604 & 0.603 & 0.534 & 0.574 & 0.552 & 0.592 & 0.602 & 0.593 & 0.618 & 0.607\\
AFA & \bfseries 0.555 & \bfseries 0.546 & \bfseries 0.634 & 0.561 & \bfseries 0.569 & \bfseries 0.582 & \bfseries 0.599 & \bfseries 0.607 & 0.670 & \bfseries 0.605 & \bfseries 0.504 & 0.652 & \bfseries 0.496 & \bfseries 0.535 & \bfseries 0.545 & \bfseries 0.607 & 0.652 & \bfseries 0.625 & \bfseries 0.586 & \bfseries 0.578 & \bfseries 0.563 & \bfseries 0.545 & 0.577 & \bfseries 0.609 & \bfseries 0.537 & \bfseries 0.545 & \bfseries 0.537 & 0.655 & \bfseries 0.507 & 0.544 & \bfseries 0.558 & 0.615 & 0.633 & \bfseries 0.541 & \bfseries 0.623 & 0.579 & 0.678 & \bfseries 0.566 & \bfseries 0.502 & 0.623 & 0.726 & 0.592 & 0.628 & \bfseries 0.583 & 0.595 & \bfseries 0.524 & \bfseries 0.525 & \bfseries 0.544 & \bfseries 0.541 & 0.585 & \bfseries 0.587 & \bfseries 0.566 & \bfseries 0.588 & \bfseries 0.582\\
\midrule
\multicolumn{55}{c}{Number of parameters = 1.6B}\\
\midrule
Baseline & 0.516 & 0.516 & 0.594 & 0.516 & 0.575 & 0.562 & 0.596 & 0.591 & \bfseries 0.577 & \bfseries 0.553 & 0.492 & 0.604 & 0.558 & 0.561 & 0.564 & 0.568 & \bfseries 0.544 & 0.581 & 0.567 & 0.617 & 0.542 & 0.549 & \bfseries 0.507 & 0.595 & 0.529 & 0.548 & 0.520 & 0.575 & 0.543 & \bfseries 0.498 & 0.570 & 0.602 & 0.575 & 0.575 & 0.575 & 0.530 & \bfseries 0.586 & 0.588 & 0.545 & 0.572 & 0.605 & \bfseries 0.516 & 0.559 & 0.567 & 0.541 & 0.525 & 0.501 & 0.522 & 0.546 & 0.508 & 0.549 & 0.550 & 0.562 & 0.555\\
BA & 0.504 & 0.534 & 0.598 & \bfseries 0.505 & 0.565 & 0.566 & 0.593 & 0.567 & 0.589 & 0.571 & 0.504 & 0.599 & 0.556 & 0.564 & 0.576 & 0.582 & 0.545 & 0.593 & 0.565 & 0.594 & 0.559 & 0.575 & 0.532 & 0.590 & 0.521 & 0.567 & 0.514 & \bfseries 0.571 & 0.539 & 0.501 & 0.571 & 0.587 & 0.570 & 0.551 & \bfseries 0.555 & \bfseries 0.515 & 0.591 & 0.589 & 0.533 & \bfseries 0.546 & \bfseries 0.597 & 0.521 & \bfseries 0.536 & 0.596 & 0.532 & 0.538 & 0.514 & 0.521 & 0.539 & 0.533 & 0.555 & 0.548 & 0.560 & 0.555\\
AFA & \bfseries 0.483 & \bfseries 0.506 & \bfseries 0.574 & 0.518 & \bfseries 0.535 & \bfseries 0.537 & \bfseries 0.556 & \bfseries 0.562 & 0.583 & 0.572 & \bfseries 0.434 & \bfseries 0.556 & \bfseries 0.486 & \bfseries 0.511 & \bfseries 0.491 & \bfseries 0.530 & 0.564 & \bfseries 0.580 & \bfseries 0.505 & \bfseries 0.525 & \bfseries 0.516 & \bfseries 0.499 & 0.514 & \bfseries 0.562 & \bfseries 0.472 & \bfseries 0.504 & \bfseries 0.456 & 0.592 & \bfseries 0.477 & 0.524 & \bfseries 0.517 & \bfseries 0.537 & \bfseries 0.564 & \bfseries 0.478 & 0.574 & 0.527 & 0.602 & \bfseries 0.515 & \bfseries 0.474 & 0.562 & 0.616 & 0.519 & 0.556 & \bfseries 0.555 & \bfseries 0.528 & \bfseries 0.481 & \bfseries 0.469 & \bfseries 0.472 & \bfseries 0.490 & \bfseries 0.507 & \bfseries 0.531 & \bfseries 0.513 & \bfseries 0.530 & \bfseries 0.525\\
\bottomrule
\end{tabular}
\caption{Language-wise results on isotropy . BA refers to Baseline adapted model. AFA refers to Active Forgetting adapted model. $\mu_\text{pretraining}$ refers to performance averaged over languages in the pretraining split. $\mu_\text{adapting}$ refers to averaging over languages in the adapting split. $\mu_\text{other}$ refers to averaging on languages that are in neither split. $\mu_\text{overall}$ refers to the average over all languages.}
\label{tab:full_isotropy}
\end{table}

==> tables/full_mlqa.tex <==
\begin{table}
\small
\centering
\begin{tabular}{lrrrrrrrrrrr}
\toprule
Model & ar & de & en & es & hi & vi & zh & $\mu_\text{pretraining}$ & $\mu_\text{adapting}$ & $\mu_\text{other}$ & $\mu_\text{overall}$ \\
\midrule
\multicolumn{12}{c}{Number of parameters = 400M}\\
\midrule
Baseline & 0.073 & 0.066 & \bfseries 0.178 & 0.084 & \bfseries 0.124 & 0.030 & 0.038 & 0.099 & N/A & 0.048 & 0.085\\
BA & 0.016 & \bfseries 0.106 & 0.131 & 0.054 & 0.041 & 0.033 & 0.051 & 0.059 & N/A & 0.069 & 0.062\\
AFA & \bfseries 0.112 & 0.067 & 0.060 & \bfseries 0.116 & 0.110 & \bfseries 0.127 & \bfseries 0.134 & \bfseries 0.106 & N/A & \bfseries 0.097 & \bfseries 0.104\\
\midrule
\multicolumn{12}{c}{Number of parameters = 782M}\\
\midrule
Baseline & \bfseries 0.142 & \bfseries 0.168 & 0.109 & 0.071 & \bfseries 0.184 & 0.092 & \bfseries 0.198 & \bfseries 0.141 & N/A & \bfseries 0.130 & \bfseries 0.138\\
BA & 0.113 & 0.067 & 0.070 & \bfseries 0.168 & 0.072 & \bfseries 0.133 & 0.135 & 0.112 & N/A & 0.100 & 0.108\\
AFA & 0.062 & 0.094 & \bfseries 0.147 & 0.071 & 0.073 & 0.093 & 0.144 & 0.099 & N/A & 0.093 & 0.098\\
\midrule
\multicolumn{12}{c}{Number of parameters = 1.6B}\\
\midrule
Baseline & \bfseries 0.180 & \bfseries 0.254 & 0.097 & 0.103 & 0.113 & \bfseries 0.243 & \bfseries 0.264 & \bfseries 0.151 & N/A & \bfseries 0.248 & \bfseries 0.179\\
BA & 0.112 & 0.106 & \bfseries 0.195 & \bfseries 0.133 & 0.055 & 0.192 & 0.198 & 0.139 & N/A & 0.149 & 0.141\\
AFA & 0.115 & 0.117 & 0.090 & 0.105 & \bfseries 0.153 & 0.089 & 0.212 & 0.135 & N/A & 0.103 & 0.126\\
\bottomrule
\end{tabular}
\caption{Language-wise results on mlqa  \citep{lewis-etal-2020-mlqa}. BA refers to Baseline adapted model. AFA refers to Active Forgetting adapted model. $\mu_\text{pretraining}$ refers to performance averaged over languages in the pretraining split. $\mu_\text{adapting}$ refers to averaging over languages in the adapting split. $\mu_\text{other}$ refers to averaging on languages that are in neither split. $\mu_\text{overall}$ refers to the average over all languages.}
\label{tab:full_mlqa}
\end{table}

==> tables/full_perplexity.tex <==
\begin{table}
\small
\centering
\begin{tabular}{lrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrr}
\toprule
Model & af & ar & az & bg & bn & co & cs & da & de & en & es & et & fi & fr & gu & ha & he & hi & hu & id & it & iw & ja & ka & ko & ml & mn & mr & my & nl & no & pl & ps & pt & ru & se & sk & sq & sr & st & sv & sw & ta & te & tg & th & tr & ur & vi & zh & $\mu_\text{pretraining}$ & $\mu_\text{adapting}$ & $\mu_\text{other}$ & $\mu_\text{overall}$ \\
\midrule
\multicolumn{55}{c}{Number of parameters = 400M}\\
\midrule
Baseline & \bfseries 29.055 & 20.523 & \bfseries 33.201 & 28.472 & 29.583 & 38.947 & \bfseries 27.003 & 31.732 & \bfseries 37.216 & \bfseries 18.006 & 34.666 & \bfseries 23.793 & \bfseries 21.030 & 31.168 & 37.239 & 35.923 & \bfseries 22.072 & 27.251 & 28.419 & 33.838 & 30.972 & 36.570 & 33.774 & 37.367 & 33.582 & \bfseries 31.753 & \bfseries 29.810 & 35.043 & \bfseries 32.258 & 34.519 & 33.268 & 28.475 & \bfseries 32.554 & \bfseries 23.639 & 25.188 & \bfseries 25.118 & 28.501 & 30.740 & 37.670 & 40.033 & 41.539 & 29.060 & \bfseries 38.312 & 39.924 & 29.268 & \bfseries 32.429 & 31.751 & 41.140 & \bfseries 38.231 & \bfseries 20.927 & \bfseries 25.041 & 31.440 & 34.663 & 31.451\\
BA & 34.999 & 21.920 & 36.702 & 33.610 & 32.229 & 37.706 & 30.790 & 31.318 & 39.029 & 19.928 & \bfseries 28.155 & 23.956 & 21.992 & 29.721 & 38.422 & \bfseries 33.995 & 23.539 & 28.156 & \bfseries 27.460 & 35.042 & \bfseries 30.846 & 38.007 & \bfseries 30.595 & 40.826 & \bfseries 33.469 & 36.558 & 35.036 & 34.875 & 37.108 & \bfseries 31.989 & \bfseries 32.274 & 26.184 & 36.076 & 23.865 & \bfseries 23.389 & 28.007 & 27.712 & 33.201 & 43.105 & \bfseries 38.779 & 42.010 & \bfseries 26.028 & 43.317 & 41.655 & 31.538 & 37.615 & 33.870 & 41.180 & 38.416 & 22.468 & 25.097 & 31.405 & 36.993 & 32.573\\
AFA & 30.549 & \bfseries 19.271 & 36.959 & \bfseries 28.024 & \bfseries 26.876 & \bfseries 34.513 & 30.568 & \bfseries 29.813 & 37.597 & 18.150 & 31.931 & 25.276 & 21.667 & \bfseries 28.564 & \bfseries 32.891 & 34.290 & 24.850 & \bfseries 25.127 & 28.791 & \bfseries 33.202 & 31.154 & \bfseries 36.437 & 32.845 & \bfseries 36.815 & 33.598 & 32.083 & 34.444 & \bfseries 32.055 & 35.581 & 33.375 & 32.442 & \bfseries 25.077 & 32.578 & 25.730 & 24.961 & 25.730 & \bfseries 27.124 & \bfseries 30.217 & \bfseries 34.922 & 39.550 & \bfseries 40.235 & 27.295 & 38.332 & \bfseries 37.967 & \bfseries 27.727 & 33.410 & \bfseries 30.900 & \bfseries 38.183 & 40.082 & 21.912 & 25.180 & \bfseries 30.373 & \bfseries 34.345 & \bfseries 31.033\\
\midrule
\multicolumn{55}{c}{Number of parameters = 782M}\\
\midrule
Baseline & \bfseries 27.111 & 18.513 & \bfseries 30.647 & 26.075 & 26.756 & 32.830 & 26.320 & 31.371 & 32.968 & 17.186 & 29.358 & \bfseries 21.109 & \bfseries 18.894 & \bfseries 26.621 & 35.473 & \bfseries 30.243 & \bfseries 21.298 & 25.584 & 29.911 & 30.936 & \bfseries 26.645 & 34.154 & 30.523 & 35.496 & 32.618 & 29.073 & \bfseries 28.579 & 32.147 & \bfseries 29.639 & 29.384 & 31.014 & 25.412 & 30.567 & \bfseries 22.757 & 24.229 & 24.081 & 25.517 & 28.105 & \bfseries 31.600 & 35.241 & 33.570 & 25.627 & 35.378 & \bfseries 33.963 & \bfseries 26.530 & 30.340 & 29.690 & 38.812 & \bfseries 32.597 & \bfseries 19.149 & 22.826 & 29.382 & 31.099 & 28.633\\
BA & 29.517 & 19.356 & 34.881 & 27.056 & 28.620 & 36.172 & \bfseries 25.525 & 30.243 & 36.159 & 17.763 & 28.108 & 22.782 & 20.519 & 27.564 & 34.371 & 32.316 & 23.137 & 24.876 & 28.308 & 33.623 & 29.027 & \bfseries 31.967 & \bfseries 28.483 & 36.059 & \bfseries 31.415 & 32.209 & 30.674 & 35.308 & 33.508 & \bfseries 28.566 & \bfseries 27.065 & 24.318 & 32.471 & 23.324 & \bfseries 21.616 & \bfseries 23.549 & 24.858 & 30.169 & 37.240 & 38.173 & 39.886 & 25.124 & 39.084 & 39.294 & 30.192 & 31.984 & 30.436 & 40.202 & 36.055 & 20.027 & 23.155 & 28.924 & 33.766 & 29.864\\
AFA & 28.498 & \bfseries 17.931 & 33.589 & \bfseries 25.051 & \bfseries 25.572 & \bfseries 30.093 & 26.629 & \bfseries 26.360 & \bfseries 32.151 & \bfseries 16.530 & \bfseries 27.865 & 23.644 & 19.090 & 27.158 & \bfseries 30.301 & 30.412 & 21.472 & \bfseries 22.964 & \bfseries 27.059 & \bfseries 29.059 & 29.808 & 35.388 & 29.836 & \bfseries 35.029 & 32.856 & \bfseries 28.789 & 30.701 & \bfseries 31.289 & 32.336 & 29.069 & 31.521 & \bfseries 21.667 & \bfseries 29.895 & 22.875 & 23.502 & 24.367 & \bfseries 23.895 & \bfseries 27.042 & 33.427 & \bfseries 32.343 & \bfseries 33.462 & \bfseries 23.824 & \bfseries 35.238 & 35.919 & 27.337 & \bfseries 28.697 & \bfseries 28.228 & \bfseries 34.969 & 34.928 & 19.468 & \bfseries 22.727 & \bfseries 27.949 & \bfseries 31.047 & \bfseries 28.183\\
\midrule
\multicolumn{55}{c}{Number of parameters = 1.6B}\\
\midrule
Baseline & 25.435 & 16.674 & \bfseries 27.741 & 24.295 & 24.641 & 30.829 & \bfseries 22.720 & 26.975 & \bfseries 29.957 & 15.194 & 27.460 & \bfseries 19.520 & 18.262 & 25.398 & 30.920 & \bfseries 28.158 & 19.550 & 23.165 & 25.076 & 27.848 & \bfseries 24.563 & 30.156 & 28.884 & \bfseries 30.084 & 28.848 & \bfseries 27.014 & \bfseries 26.108 & 30.317 & \bfseries 28.617 & 27.681 & 28.592 & 22.651 & \bfseries 27.323 & 21.114 & 21.161 & 22.233 & 23.013 & \bfseries 26.043 & 30.484 & \bfseries 31.465 & 32.448 & 22.808 & 32.242 & 31.479 & 24.176 & 28.721 & 28.229 & \bfseries 32.626 & 31.745 & 17.864 & 20.745 & 26.831 & 28.497 & 26.170\\
BA & 27.832 & 17.335 & 29.341 & 26.423 & 26.509 & 33.171 & 24.139 & 26.689 & 31.339 & 16.138 & \bfseries 24.868 & 19.656 & 18.547 & 23.909 & 32.046 & 29.106 & 20.544 & 23.945 & 24.366 & 29.716 & 25.020 & 31.496 & \bfseries 26.220 & 32.588 & \bfseries 27.614 & 29.152 & 28.684 & 31.059 & 31.019 & 25.999 & \bfseries 25.894 & 21.027 & 30.527 & 20.825 & \bfseries 19.476 & 21.794 & 24.446 & 27.740 & 33.686 & 34.932 & 34.877 & \bfseries 21.190 & 34.662 & 34.205 & 26.747 & 30.096 & 28.101 & 33.865 & 32.712 & 19.084 & 20.828 & 26.117 & 30.616 & 27.007\\
AFA & \bfseries 23.682 & \bfseries 16.119 & 29.057 & \bfseries 22.052 & \bfseries 23.272 & \bfseries 29.596 & 23.798 & \bfseries 24.672 & 31.395 & \bfseries 14.516 & 27.263 & 20.322 & \bfseries 18.206 & \bfseries 23.153 & \bfseries 28.601 & 29.425 & \bfseries 19.543 & \bfseries 22.116 & \bfseries 23.848 & \bfseries 26.686 & 25.663 & \bfseries 29.833 & 28.146 & 31.498 & 27.653 & 28.158 & 27.329 & \bfseries 27.981 & 28.640 & \bfseries 25.774 & 26.214 & \bfseries 20.565 & 27.942 & \bfseries 20.435 & 20.661 & \bfseries 20.280 & \bfseries 22.493 & 26.217 & \bfseries 29.691 & 31.866 & \bfseries 32.374 & 21.799 & \bfseries 30.796 & \bfseries 30.247 & \bfseries 24.078 & \bfseries 26.352 & \bfseries 26.995 & 33.400 & \bfseries 31.528 & \bfseries 17.843 & \bfseries 20.654 & \bfseries 25.048 & \bfseries 28.386 & \bfseries 25.596\\
\bottomrule
\end{tabular}
\caption{Language-wise results on perplexity . BA refers to Baseline adapted model. AFA refers to Active Forgetting adapted model. $\mu_\text{pretraining}$ refers to performance averaged over languages in the pretraining split. $\mu_\text{adapting}$ refers to averaging over languages in the adapting split. $\mu_\text{other}$ refers to averaging on languages that are in neither split. $\mu_\text{overall}$ refers to the average over all languages.}
\label{tab:full_perplexity}
\end{table}

==> tables/full_translation.tex <==
\begin{table}
\small
\centering
\begin{tabular}{lrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrr}
\toprule
Model & af & ar & az & bg & bn & co & cs & da & de & en & es & et & fi & fr & gu & ha & he & hi & hu & id & it & iw & ja & ka & ko & ml & mn & mr & my & nl & no & pl & ps & pt & ru & se & sk & sq & sr & st & sv & sw & ta & te & tg & th & tr & ur & vi & zh & $\mu_\text{pretraining}$ & $\mu_\text{adapting}$ & $\mu_\text{other}$ & $\mu_\text{overall}$ \\
\midrule
\multicolumn{55}{c}{Number of parameters = 400M}\\
\midrule
Baseline & 0.105 & \bfseries 0.150 & \bfseries 0.118 & 0.058 & \bfseries 0.199 & \bfseries 0.129 & 0.074 & 0.098 & 0.078 & 0.073 & 0.056 & 0.080 & \bfseries 0.171 & 0.074 & 0.050 & 0.077 & 0.081 & 0.046 & 0.070 & \bfseries 0.151 & 0.036 & \bfseries 0.067 & 0.053 & 0.072 & 0.135 & 0.070 & 0.112 & 0.073 & 0.040 & 0.084 & \bfseries 0.110 & 0.071 & 0.075 & 0.075 & 0.074 & 0.060 & \bfseries 0.140 & 0.094 & \bfseries 0.192 & \bfseries 0.102 & 0.057 & 0.045 & \bfseries 0.148 & 0.054 & \bfseries 0.161 & 0.041 & \bfseries 0.180 & 0.036 & 0.058 & 0.075 & 0.080 & 0.084 & \bfseries 0.100 & 0.091\\
BA & 0.073 & 0.086 & 0.115 & 0.048 & 0.050 & 0.092 & 0.081 & 0.063 & \bfseries 0.137 & \bfseries 0.118 & \bfseries 0.088 & \bfseries 0.142 & 0.157 & \bfseries 0.112 & \bfseries 0.101 & \bfseries 0.142 & 0.091 & \bfseries 0.073 & 0.068 & 0.025 & \bfseries 0.073 & 0.025 & \bfseries 0.141 & \bfseries 0.115 & 0.065 & 0.062 & 0.103 & \bfseries 0.090 & \bfseries 0.152 & 0.080 & 0.070 & \bfseries 0.129 & 0.044 & \bfseries 0.131 & \bfseries 0.101 & \bfseries 0.076 & 0.063 & 0.030 & 0.042 & 0.063 & 0.049 & \bfseries 0.055 & 0.077 & 0.048 & 0.031 & 0.090 & 0.077 & 0.032 & \bfseries 0.162 & \bfseries 0.151 & \bfseries 0.101 & 0.092 & 0.074 & 0.086\\
AFA & \bfseries 0.118 & 0.061 & 0.076 & \bfseries 0.159 & 0.057 & 0.104 & \bfseries 0.083 & \bfseries 0.112 & 0.074 & 0.062 & 0.059 & 0.130 & 0.071 & 0.108 & 0.062 & 0.098 & \bfseries 0.116 & 0.026 & \bfseries 0.070 & 0.061 & 0.068 & 0.053 & 0.039 & 0.066 & \bfseries 0.211 & \bfseries 0.097 & \bfseries 0.149 & 0.072 & 0.076 & \bfseries 0.221 & 0.089 & 0.035 & \bfseries 0.162 & 0.108 & 0.085 & 0.073 & 0.100 & \bfseries 0.109 & 0.108 & 0.069 & \bfseries 0.138 & 0.039 & 0.049 & \bfseries 0.076 & 0.109 & \bfseries 0.165 & 0.077 & \bfseries 0.088 & 0.145 & 0.138 & 0.078 & \bfseries 0.103 & 0.098 & \bfseries 0.094\\
\midrule
\multicolumn{55}{c}{Number of parameters = 782M}\\
\midrule
Baseline & \bfseries 0.136 & \bfseries 0.215 & 0.186 & 0.153 & 0.131 & \bfseries 0.220 & 0.075 & 0.094 & 0.104 & 0.146 & 0.088 & \bfseries 0.095 & \bfseries 0.186 & 0.186 & 0.076 & \bfseries 0.186 & \bfseries 0.210 & \bfseries 0.247 & 0.154 & 0.131 & \bfseries 0.174 & 0.095 & 0.111 & \bfseries 0.234 & 0.210 & 0.209 & 0.173 & 0.224 & 0.086 & 0.111 & 0.098 & 0.105 & 0.081 & 0.189 & \bfseries 0.172 & 0.098 & 0.117 & 0.194 & \bfseries 0.182 & 0.076 & \bfseries 0.200 & 0.144 & \bfseries 0.220 & 0.101 & \bfseries 0.177 & 0.146 & 0.135 & \bfseries 0.207 & 0.107 & \bfseries 0.193 & \bfseries 0.162 & 0.138 & 0.154 & 0.152\\
BA & 0.073 & 0.126 & 0.074 & 0.126 & 0.081 & 0.096 & 0.072 & \bfseries 0.264 & 0.098 & 0.157 & 0.172 & 0.089 & 0.179 & \bfseries 0.291 & \bfseries 0.245 & 0.125 & 0.154 & 0.062 & 0.116 & \bfseries 0.157 & 0.174 & 0.094 & 0.139 & 0.099 & \bfseries 0.278 & 0.205 & 0.126 & 0.124 & \bfseries 0.159 & \bfseries 0.243 & \bfseries 0.193 & 0.118 & 0.121 & \bfseries 0.307 & 0.156 & 0.112 & 0.088 & 0.146 & 0.128 & 0.122 & 0.082 & 0.065 & 0.155 & 0.083 & 0.153 & \bfseries 0.221 & \bfseries 0.268 & 0.174 & 0.082 & 0.110 & 0.127 & \bfseries 0.208 & 0.119 & 0.146\\
AFA & 0.135 & 0.198 & \bfseries 0.243 & \bfseries 0.222 & \bfseries 0.251 & 0.202 & \bfseries 0.203 & 0.178 & \bfseries 0.162 & \bfseries 0.190 & \bfseries 0.205 & 0.090 & 0.180 & 0.189 & 0.202 & 0.130 & 0.136 & 0.134 & \bfseries 0.184 & 0.084 & 0.172 & \bfseries 0.231 & \bfseries 0.203 & 0.161 & 0.220 & \bfseries 0.251 & \bfseries 0.192 & \bfseries 0.288 & 0.112 & 0.112 & 0.184 & \bfseries 0.145 & \bfseries 0.131 & 0.245 & 0.155 & \bfseries 0.127 & \bfseries 0.216 & \bfseries 0.232 & 0.152 & \bfseries 0.153 & 0.158 & \bfseries 0.150 & 0.216 & \bfseries 0.169 & 0.142 & 0.173 & 0.215 & 0.130 & \bfseries 0.252 & 0.085 & 0.158 & 0.190 & \bfseries 0.180 & \bfseries 0.178\\
\midrule
\multicolumn{55}{c}{Number of parameters = 1.6B}\\
\midrule
Baseline & 0.175 & \bfseries 0.278 & 0.164 & \bfseries 0.261 & \bfseries 0.178 & \bfseries 0.249 & \bfseries 0.234 & 0.187 & \bfseries 0.274 & 0.214 & 0.127 & 0.166 & 0.157 & 0.179 & 0.297 & \bfseries 0.280 & \bfseries 0.276 & \bfseries 0.223 & 0.114 & \bfseries 0.207 & 0.243 & 0.265 & 0.162 & 0.228 & 0.281 & \bfseries 0.295 & \bfseries 0.271 & 0.270 & \bfseries 0.282 & 0.109 & 0.185 & 0.159 & \bfseries 0.191 & 0.237 & 0.127 & 0.208 & 0.145 & \bfseries 0.278 & \bfseries 0.214 & 0.104 & \bfseries 0.221 & \bfseries 0.291 & 0.178 & \bfseries 0.233 & 0.115 & 0.222 & 0.140 & \bfseries 0.227 & 0.264 & 0.164 & \bfseries 0.208 & 0.197 & \bfseries 0.221 & 0.211\\
BA & 0.114 & 0.184 & 0.124 & 0.187 & 0.128 & 0.130 & 0.097 & \bfseries 0.293 & 0.138 & 0.095 & 0.090 & 0.093 & 0.139 & 0.201 & \bfseries 0.359 & 0.168 & 0.088 & 0.157 & \bfseries 0.340 & 0.074 & 0.167 & 0.181 & \bfseries 0.195 & 0.118 & \bfseries 0.319 & 0.144 & 0.187 & \bfseries 0.341 & 0.109 & \bfseries 0.289 & 0.133 & 0.199 & 0.155 & 0.301 & 0.176 & \bfseries 0.236 & 0.157 & 0.182 & 0.170 & 0.114 & 0.180 & 0.121 & 0.094 & 0.144 & \bfseries 0.196 & \bfseries 0.334 & 0.298 & 0.163 & 0.178 & 0.202 & 0.134 & \bfseries 0.274 & 0.147 & 0.180\\
AFA & \bfseries 0.278 & 0.133 & \bfseries 0.211 & 0.189 & 0.147 & 0.193 & 0.102 & 0.165 & 0.228 & \bfseries 0.243 & \bfseries 0.176 & \bfseries 0.170 & \bfseries 0.232 & \bfseries 0.330 & 0.327 & 0.196 & 0.252 & 0.114 & 0.258 & 0.144 & \bfseries 0.295 & \bfseries 0.278 & 0.139 & \bfseries 0.308 & 0.267 & 0.128 & 0.265 & 0.236 & 0.135 & 0.208 & \bfseries 0.367 & \bfseries 0.225 & 0.165 & \bfseries 0.361 & \bfseries 0.257 & 0.217 & \bfseries 0.180 & 0.218 & 0.206 & \bfseries 0.145 & 0.120 & 0.244 & \bfseries 0.264 & 0.137 & 0.151 & 0.148 & \bfseries 0.308 & 0.163 & \bfseries 0.295 & \bfseries 0.212 & 0.202 & 0.254 & 0.198 & \bfseries 0.215\\
\bottomrule
\end{tabular}
\caption{Language-wise results on translation  (en-to-XX) on the subset of languages from FLORES-200 \citep{nllb-22}. BA refers to Baseline adapted model. AFA refers to Active Forgetting adapted model. $\mu_\text{pretraining}$ refers to performance averaged over languages in the pretraining split. $\mu_\text{adapting}$ refers to averaging over languages in the adapting split. $\mu_\text{other}$ refers to averaging on languages that are in neither split. $\mu_\text{overall}$ refers to the average over all languages.}
\label{tab:full_translation}
\end{table}

==> tables/full_xcopa.tex <==
\begin{table}
\small
\centering
\begin{tabular}{lrrrrrrrrrrrrrrr}
\toprule
Model & et & ht & id & it & qu & sw & ta & th & tr & vi & zh & $\mu_\text{pretraining}$ & $\mu_\text{adapting}$ & $\mu_\text{other}$ & $\mu_\text{overall}$ \\
\midrule
\multicolumn{16}{c}{Number of parameters = 400M}\\
\midrule
Baseline & \bfseries 0.176 & \bfseries 0.147 & \bfseries 0.108 & 0.103 & \bfseries 0.144 & \bfseries 0.140 & 0.068 & 0.148 & 0.074 & 0.066 & 0.105 & \bfseries 0.131 & 0.111 & 0.107 & 0.116\\
BA & 0.054 & 0.076 & 0.098 & 0.094 & 0.088 & 0.084 & 0.059 & \bfseries 0.182 & 0.115 & 0.119 & \bfseries 0.113 & 0.086 & 0.149 & 0.088 & 0.098\\
AFA & 0.159 & 0.103 & 0.067 & \bfseries 0.130 & 0.120 & 0.056 & \bfseries 0.115 & 0.140 & \bfseries 0.188 & \bfseries 0.146 & 0.102 & 0.112 & \bfseries 0.164 & \bfseries 0.110 & \bfseries 0.121\\
\midrule
\multicolumn{16}{c}{Number of parameters = 782M}\\
\midrule
Baseline & 0.212 & \bfseries 0.231 & 0.172 & \bfseries 0.244 & 0.231 & \bfseries 0.256 & 0.189 & 0.251 & 0.156 & \bfseries 0.197 & \bfseries 0.197 & \bfseries 0.227 & 0.204 & 0.204 & 0.212\\
BA & 0.187 & 0.142 & 0.133 & 0.146 & 0.208 & 0.138 & 0.149 & 0.216 & \bfseries 0.228 & 0.138 & 0.173 & 0.161 & 0.222 & 0.154 & 0.169\\
AFA & \bfseries 0.232 & 0.208 & \bfseries 0.233 & 0.234 & \bfseries 0.237 & 0.217 & \bfseries 0.214 & \bfseries 0.285 & 0.206 & 0.189 & 0.193 & 0.219 & \bfseries 0.245 & \bfseries 0.216 & \bfseries 0.223\\
\midrule
\multicolumn{16}{c}{Number of parameters = 1.6B}\\
\midrule
Baseline & 0.258 & 0.211 & 0.256 & 0.200 & 0.261 & \bfseries 0.246 & \bfseries 0.299 & 0.279 & 0.271 & \bfseries 0.286 & \bfseries 0.247 & 0.238 & 0.275 & 0.263 & 0.256\\
BA & 0.202 & 0.170 & 0.207 & 0.178 & 0.199 & 0.196 & 0.262 & \bfseries 0.368 & 0.270 & 0.212 & 0.223 & 0.200 & 0.319 & 0.210 & 0.226\\
AFA & \bfseries 0.289 & \bfseries 0.223 & \bfseries 0.316 & \bfseries 0.278 & \bfseries 0.266 & 0.239 & 0.265 & 0.301 & \bfseries 0.340 & 0.245 & 0.209 & \bfseries 0.254 & \bfseries 0.321 & \bfseries 0.263 & \bfseries 0.270\\
\bottomrule
\end{tabular}
\caption{Language-wise results on xcopa  \citep{ponti-etal-2020-xcopa}. BA refers to Baseline adapted model. AFA refers to Active Forgetting adapted model. $\mu_\text{pretraining}$ refers to performance averaged over languages in the pretraining split. $\mu_\text{adapting}$ refers to averaging over languages in the adapting split. $\mu_\text{other}$ refers to averaging on languages that are in neither split. $\mu_\text{overall}$ refers to the average over all languages.}
\label{tab:full_xcopa}
\end{table}

==> tables/full_xlsum.tex <==
\begin{table}
\small
\centering
\begin{tabular}{lrrrrrrrrrrr}
\toprule
Model & ar & en & es & fr & hi & jp & zh & $\mu_\text{pretraining}$ & $\mu_\text{adapting}$ & $\mu_\text{other}$ & $\mu_\text{overall}$ \\
\midrule
\multicolumn{12}{c}{Number of parameters = 400M}\\
\midrule
Baseline & 0.058 & 0.060 & \bfseries 0.036 & 0.031 & \bfseries 0.086 & 0.037 & 0.058 & \bfseries 0.060 & 0.031 & 0.037 & 0.052\\
BA & 0.037 & 0.069 & 0.027 & 0.024 & 0.027 & \bfseries 0.054 & 0.034 & 0.039 & 0.024 & \bfseries 0.054 & 0.039\\
AFA & \bfseries 0.063 & \bfseries 0.070 & 0.033 & \bfseries 0.095 & 0.053 & 0.048 & \bfseries 0.061 & 0.056 & \bfseries 0.095 & 0.048 & \bfseries 0.060\\
\midrule
\multicolumn{12}{c}{Number of parameters = 782M}\\
\midrule
Baseline & \bfseries 0.084 & \bfseries 0.091 & \bfseries 0.074 & 0.074 & \bfseries 0.089 & 0.084 & 0.087 & \bfseries 0.085 & 0.074 & 0.084 & 0.083\\
BA & 0.054 & 0.043 & 0.055 & 0.100 & 0.056 & 0.052 & 0.069 & 0.055 & 0.100 & 0.052 & 0.061\\
AFA & 0.069 & 0.058 & 0.057 & \bfseries 0.113 & 0.087 & \bfseries 0.095 & \bfseries 0.108 & 0.076 & \bfseries 0.113 & \bfseries 0.095 & \bfseries 0.084\\
\midrule
\multicolumn{12}{c}{Number of parameters = 1.6B}\\
\midrule
Baseline & \bfseries 0.109 & \bfseries 0.094 & \bfseries 0.093 & 0.119 & 0.086 & \bfseries 0.110 & 0.096 & 0.096 & 0.119 & \bfseries 0.110 & 0.101\\
BA & 0.063 & 0.094 & 0.072 & 0.115 & 0.071 & 0.058 & 0.080 & 0.076 & 0.115 & 0.058 & 0.079\\
AFA & 0.104 & 0.089 & 0.078 & \bfseries 0.134 & \bfseries 0.093 & 0.109 & \bfseries 0.121 & \bfseries 0.097 & \bfseries 0.134 & 0.109 & \bfseries 0.104\\
\bottomrule
\end{tabular}
\caption{Language-wise results on xlsum  \citep{hasan-etal-2021-xl}. BA refers to Baseline adapted model. AFA refers to Active Forgetting adapted model. $\mu_\text{pretraining}$ refers to performance averaged over languages in the pretraining split. $\mu_\text{adapting}$ refers to averaging over languages in the adapting split. $\mu_\text{other}$ refers to averaging on languages that are in neither split. $\mu_\text{overall}$ refers to the average over all languages.}
\label{tab:full_xlsum}
\end{table}

==> tables/full_xnli.tex <==
\begin{table}
\small
\centering
\begin{tabular}{lrrrrrrrrrrrrrrr}
\toprule
Model & et & ht & id & it & qu & sw & ta & th & tr & vi & zh & $\mu_\text{pretraining}$ & $\mu_\text{adapting}$ & $\mu_\text{other}$ & $\mu_\text{overall}$ \\
\midrule
\multicolumn{16}{c}{Number of parameters = 400M}\\
\midrule
Baseline & 0.033 & 0.059 & 0.053 & 0.038 & 0.086 & \bfseries 0.145 & \bfseries 0.124 & 0.081 & 0.115 & \bfseries 0.103 & 0.058 & 0.068 & 0.098 & 0.085 & 0.081\\
BA & 0.052 & 0.075 & 0.080 & 0.060 & 0.022 & 0.057 & 0.054 & 0.127 & 0.110 & 0.069 & \bfseries 0.127 & 0.074 & 0.118 & 0.060 & 0.076\\
AFA & \bfseries 0.085 & \bfseries 0.138 & \bfseries 0.102 & \bfseries 0.094 & \bfseries 0.112 & 0.075 & 0.069 & \bfseries 0.139 & \bfseries 0.207 & 0.064 & 0.093 & \bfseries 0.087 & \bfseries 0.173 & \bfseries 0.097 & \bfseries 0.107\\
\midrule
\multicolumn{16}{c}{Number of parameters = 782M}\\
\midrule
Baseline & 0.129 & 0.095 & 0.065 & \bfseries 0.163 & 0.064 & 0.170 & 0.086 & 0.084 & 0.140 & 0.110 & \bfseries 0.201 & \bfseries 0.166 & 0.112 & 0.084 & 0.119\\
BA & \bfseries 0.153 & 0.074 & 0.079 & 0.080 & 0.056 & \bfseries 0.170 & 0.072 & 0.208 & \bfseries 0.189 & \bfseries 0.129 & 0.090 & 0.123 & \bfseries 0.198 & 0.082 & 0.118\\
AFA & 0.088 & \bfseries 0.133 & \bfseries 0.190 & 0.102 & \bfseries 0.084 & 0.138 & \bfseries 0.169 & \bfseries 0.247 & 0.141 & 0.063 & 0.121 & 0.112 & 0.194 & \bfseries 0.128 & \bfseries 0.134\\
\midrule
\multicolumn{16}{c}{Number of parameters = 1.6B}\\
\midrule
Baseline & 0.120 & \bfseries 0.236 & 0.148 & \bfseries 0.252 & 0.181 & \bfseries 0.133 & 0.171 & 0.199 & 0.134 & 0.117 & 0.179 & 0.171 & 0.167 & 0.171 & 0.170\\
BA & 0.107 & 0.192 & 0.096 & 0.180 & \bfseries 0.200 & 0.095 & \bfseries 0.216 & 0.111 & 0.225 & 0.150 & 0.118 & 0.125 & 0.168 & \bfseries 0.171 & 0.154\\
AFA & \bfseries 0.166 & 0.095 & \bfseries 0.183 & 0.210 & 0.130 & 0.099 & 0.180 & \bfseries 0.363 & \bfseries 0.257 & \bfseries 0.186 & \bfseries 0.293 & \bfseries 0.192 & \bfseries 0.310 & 0.155 & \bfseries 0.197\\
\bottomrule
\end{tabular}
\caption{Language-wise results on xnli  \citep{conneau-etal-2018-xnli}. BA refers to Baseline adapted model. AFA refers to Active Forgetting adapted model. $\mu_\text{pretraining}$ refers to performance averaged over languages in the pretraining split. $\mu_\text{adapting}$ refers to averaging over languages in the adapting split. $\mu_\text{other}$ refers to averaging on languages that are in neither split. $\mu_\text{overall}$ refers to the average over all languages.}
\label{tab:full_xnli}
\end{table}

==> tables/full_xquad.tex <==
\begin{table}
\small
\centering
\begin{tabular}{lrrrrrrrrrrrrrrrr}
\toprule
Model & ar & de & el & en & es & hi & ro & ru & th & tr & vi & zh & $\mu_\text{pretraining}$ & $\mu_\text{adapting}$ & $\mu_\text{other}$ & $\mu_\text{overall}$ \\
\midrule
\multicolumn{17}{c}{Number of parameters = 400M}\\
\midrule
Baseline & \bfseries 0.119 & 0.077 & \bfseries 0.134 & \bfseries 0.161 & \bfseries 0.174 & 0.077 & \bfseries 0.115 & \bfseries 0.126 & 0.055 & 0.173 & 0.066 & \bfseries 0.170 & \bfseries 0.138 & 0.114 & 0.098 & \bfseries 0.121\\
BA & 0.048 & \bfseries 0.163 & 0.063 & 0.113 & 0.082 & 0.090 & 0.104 & 0.118 & 0.199 & 0.156 & \bfseries 0.086 & 0.104 & 0.093 & 0.178 & \bfseries 0.104 & 0.111\\
AFA & 0.095 & 0.073 & 0.058 & 0.079 & 0.079 & \bfseries 0.104 & 0.108 & 0.064 & \bfseries 0.243 & \bfseries 0.222 & 0.070 & 0.154 & 0.096 & \bfseries 0.233 & 0.077 & 0.112\\
\midrule
\multicolumn{17}{c}{Number of parameters = 782M}\\
\midrule
Baseline & \bfseries 0.206 & \bfseries 0.260 & 0.179 & 0.175 & \bfseries 0.213 & 0.156 & \bfseries 0.235 & 0.188 & 0.179 & 0.190 & 0.178 & \bfseries 0.180 & 0.186 & 0.185 & \bfseries 0.213 & 0.195\\
BA & 0.126 & 0.132 & 0.144 & 0.132 & 0.139 & 0.174 & 0.158 & 0.152 & 0.197 & \bfseries 0.253 & 0.147 & 0.157 & 0.147 & \bfseries 0.225 & 0.145 & 0.159\\
AFA & 0.135 & 0.215 & \bfseries 0.231 & \bfseries 0.183 & 0.204 & \bfseries 0.247 & 0.182 & \bfseries 0.221 & \bfseries 0.207 & 0.228 & \bfseries 0.215 & 0.155 & \bfseries 0.191 & 0.218 & 0.211 & \bfseries 0.202\\
\midrule
\multicolumn{17}{c}{Number of parameters = 1.6B}\\
\midrule
Baseline & 0.233 & 0.256 & 0.215 & 0.225 & \bfseries 0.241 & \bfseries 0.291 & 0.230 & \bfseries 0.242 & 0.216 & 0.280 & 0.223 & 0.228 & \bfseries 0.243 & 0.248 & 0.231 & 0.240\\
BA & \bfseries 0.239 & 0.216 & 0.243 & 0.178 & 0.190 & 0.179 & 0.215 & 0.173 & 0.251 & 0.319 & 0.191 & 0.212 & 0.195 & 0.285 & 0.216 & 0.217\\
AFA & 0.238 & \bfseries 0.283 & \bfseries 0.247 & \bfseries 0.291 & 0.219 & 0.249 & \bfseries 0.239 & 0.205 & \bfseries 0.341 & \bfseries 0.329 & \bfseries 0.266 & \bfseries 0.252 & 0.242 & \bfseries 0.335 & \bfseries 0.258 & \bfseries 0.263\\
\bottomrule
\end{tabular}
\caption{Language-wise results on xquad  \citep{artetxe-etal-2020-cross}. BA refers to Baseline adapted model. AFA refers to Active Forgetting adapted model. $\mu_\text{pretraining}$ refers to performance averaged over languages in the pretraining split. $\mu_\text{adapting}$ refers to averaging over languages in the adapting split. $\mu_\text{other}$ refers to averaging on languages that are in neither split. $\mu_\text{overall}$ refers to the average over all languages.}
\label{tab:full_xquad}
\end{table}

==> tables/short_xnli.tex <==
\begin{table}
\small
\centering
\begin{tabular}{lrrrr}
\toprule
Model & $\mu_\text{pretraining}$ & $\mu_\text{adapting}$ & $\mu_\text{other}$ & $\mu_\text{overall}$ \\
\midrule
\multicolumn{5}{c}{Number of parameters = 400M}\\
\midrule
Baseline & 0.068 & 0.098 & 0.085 & 0.081\\
BA & 0.074 & 0.118 & 0.060 & 0.076\\
AFA & \bfseries 0.087 & \bfseries 0.173 & \bfseries 0.097 & \bfseries 0.107\\
\midrule
\multicolumn{5}{c}{Number of parameters = 782M}\\
\midrule
Baseline & \bfseries 0.166 & 0.112 & 0.084 & 0.119\\
BA & 0.123 & \bfseries 0.198 & 0.082 & 0.118\\
AFA & 0.112 & 0.194 & \bfseries 0.128 & \bfseries 0.134\\
\midrule
\multicolumn{5}{c}{Number of parameters = 1.6B}\\
\midrule
Baseline & 0.171 & 0.167 & 0.171 & 0.170\\
BA & 0.125 & 0.168 & \bfseries 0.171 & 0.154\\
AFA & \bfseries 0.192 & \bfseries 0.310 & 0.155 & \bfseries 0.197\\
\bottomrule
\end{tabular}
\caption{Detailed results on xnli \citep{conneau-etal-2018-xnli}. BA refers to Baseline adapted model. AFA refers to Active Forgetting adapted model. $\mu_\text{pretraining}$ refers to performance averaged over languages in the pretraining split. $\mu_\text{adapting}$ refers to averaging over languages in the adapting split. $\mu_\text{other}$ refers to averaging on languages that are in neither split. $\mu_\text{overall}$ refers to the average over all languages.}
\label{tab:short_xnli}
\end{table}
